Social Practice Cards: Research material to study social contexts as interwoven practice constellations

Studying how social contexts shape technology interactions and how we experience them is hard. One challenge is that social contexts are very dynamic and shaped by the situated practices of everyone involved. As a result, the same human-technology interaction can be experienced quite differently depending on what other people around us do. As a first step to study interpersonal and interpractice dynamics, we collected a broad range of visual representations of practices, such as "riding a bike" or "skipping the rope". This material can be used to further explore how different, co-located practices relate to each other.

==> CHI'22 Workshop/figures/categories.tex <==
\begin{table}[h]
  \caption{Categorization of Silhouettes according to some formal criteria. At
  the bottom of the table we have included summaries for each criterion.}
  \label{tab:categories}
  \begin{tabular}{lllc}
    \toprule
    Performers & Posture  & Group  & Silhouettes \\
    \midrule
    alone      & lying    & child  &   2 \\
    alone      & lying    & female &   2 \\
    alone      & lying    & male   &   2 \\
    alone      & sitting  & child  &   2 \\
    alone      & sitting  & female &  11 \\
    alone      & sitting  & male   &   7 \\
    alone      & standing & child  &   4 \\
    alone      & standing & female &  12 \\
    alone      & standing & male   &  27 \\
    alone      & moving   & child  &   9 \\
    alone      & moving   & female &  23 \\
    alone      & moving   & male   &  33 \\
    alone      & other    & female &   1 \\
    together   & dynamic  & child  &   7 \\
    together   & dynamic  & female &   5 \\
    together   & dynamic  & mixed  &  29 \\
    together   & static   & child  &   3 \\
    together   & static   & female &   2 \\
    together   & static   & male   &   7 \\
    together   & static   & mixed  &  13 \\
    together   & mixed    & mixed  &   1 \\
    technology &          &        &   1 \\[0.1in]
    child      &          &        &  27 \\
    female     &          &        &  56 \\
    male       &          &        &  76 \\
    mixed      &          &        &  43 \\[0.1in]
    alone      &          &        & 135 \\
    together   &          &        &  67 \\[0.1in]
    lying      &          &        &   6 \\
    sitting    &          &        &  20 \\
    standing   &          &        &  43 \\
    moving     &          &        &  65 \\
    dynamic    &          &        &  41 \\
    static     &          &        &  25 \\
  \bottomrule
\end{tabular}
\end{table}

